Regularization methods for the short-term forecasting of the Italian electric load

The problem of forecasting the whole 24 profile of the Italian electric load is addressed as a multitask learning problem, whose complexity is kept under control via alternative regularization methods. In view of the quarter-hourly samplings, 96 predictors are used, each of which linearly depends on 96 regressors. The 96x96 matrix weights form a 96x96 matrix, that can be seen and displayed as a surface sampled on a square domain. Different regularization and sparsity approaches to reduce the degrees of freedom of the surface were explored, comparing the obtained forecasts with those of the Italian Transmission System Operator Terna. Besides outperforming Terna in terms of quarter-hourly mean absolute percentage error and mean absolute error, the prediction residuals turned out to be weakly correlated with Terna, which suggests that further improvement could ensue from forecasts aggregation. In fact, the aggregated forecasts yielded further relevant drops in terms of quarter-hourly and daily mean absolute percentage error, mean absolute error and root mean square error (up to 30%) over the three test years considered.

==> paper SETA/Table1.tex <==
\begin{table*}[!ht]
\caption{Hyperparameters tuning: cross-validation results}
\centering
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{ TA }} & \multirow{3}{*}{\thead{ TS }} & \multirow{3}{*}{\thead{  RBF  }} & \multirow{3}{*}{\thead{TE}} & \multirow{3}{*}{\thead{OnE}}  \\
& & & & & \\
& & & & & \\
\hline
\multirow{3}{*}{\thead{Train: 2015 \\ Val: 2016}} & \multirow{3}{*}{$\lambda=0.1$} & \multirow{2}{*}{$\lambda_1=10$} & \multirow{3}{*}{$\lambda=1$} & \multirow{2}{*}{$\lambda_{diag}=0.01$} & \multirow{3}{*}{$\lambda_{diag}=100$}  \\ 
& & \multirow{2}{*}{$\lambda_2=100$} & & \multirow{2}{*}{$\lambda_{last}=100$} & \\
& & & & & \\
\hline
\multirow{3}{*}{\thead{Train: 2016 \\ Val: 2017}} & \multirow{3}{*}{$\lambda=0.1$} & \multirow{2}{*}{$\lambda_1=10$} & \multirow{3}{*}{$\lambda=10$} & \multirow{2}{*}{$\lambda_{diag}=1$} & \multirow{3}{*}{$\lambda_{diag}=10000$}  \\
& & \multirow{2}{*}{$\lambda_2=1$} & & \multirow{2}{*}{$\lambda_{last}=0.01$} & \\
& & & & & \\
\hline
\multirow{3}{*}{\thead{Train: 2017 \\ Val: 2018}} & \multirow{3}{*}{$\lambda=1$} & \multirow{2}{*}{$\lambda_1=100$} & \multirow{3}{*}{$\lambda=10$} & \multirow{2}{*}{$\lambda_{diag}=0.01$} & \multirow{3}{*}{$\lambda_{diag}=10000$}  \\
& & \multirow{2}{*}{$\lambda_2=10$} & & \multirow{2}{*}{$\lambda_{last}=1$} & \\
& & & & & \\
\hline
\end{tabular}%
}
\label{table:Table1}
\end{table*}

==> paper SETA/Table2.tex <==
\begin{table*}[!htb]
\caption{Forecast performances on 2017, with the percentage variation with respect to Terna results between brackets.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{MAPE [\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAPE_{daily}[\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{dof}$}} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{Terna}} & \multirow{3}{*}{$2.16$} & \multirow{3}{*}{$\bf{1.06}$} & \multirow{3}{*}{$0.83$} & \multirow{3}{*}{$\bf{1.22}$} & \multirow{3}{*}{$\bf{0.62}$} & \multirow{3}{*}{$\bf{0.47}$} & \multirow{3}{*}{Unknown} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{OLS}} & \multirow{3}{*}{$2.63\;(22\%)$} & \multirow{3}{*}{$1.41\;(33\%)$} & \multirow{3}{*}{$1.01\;(22\%)$} & \multirow{3}{*}{$1.86\;(52\%)$} & \multirow{3}{*}{$0.95\;(53\%)$} & \multirow{3}{*}{$0.69\;(47\%)$} & \multirow{3}{*}{$9216$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TA}} & \multirow{3}{*}{$1.97\;(-9\%)$} & \multirow{3}{*}{$1.07\;(1\%)$} & \multirow{3}{*}{$0.75\;(-10\%)$} & \multirow{3}{*}{$1.42\;(16\%)$} & \multirow{3}{*}{$0.73\;(18\%)$} & \multirow{3}{*}{$0.53\;(13\%)$} & \multirow{3}{*}{$1686.12$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TS}} & \multirow{3}{*}{$1.97\;(-9\%)$} & \multirow{3}{*}{$1.07\;(1\%)$} & \multirow{3}{*}{$0.76\;(-8\%)$} & \multirow{3}{*}{$1.41\;(16\%)$} & \multirow{3}{*}{$0.73\;(18\%)$} & \multirow{3}{*}{$0.53\;(13\%)$} & \multirow{3}{*}{$138.38$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{RBF}} & \multirow{3}{*}{$\bf{1.97\;(-9\%)}$} & \multirow{3}{*}{$1.08\;(2\%)$} & \multirow{3}{*}{$\bf{0.76\;(-8\%)}$} & \multirow{3}{*}{$1.43\;(17\%)$} & \multirow{3}{*}{$0.73\;(18\%)$} & \multirow{3}{*}{$0.54\;(15\%)$} & \multirow{3}{*}{$132.88$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TE}} & \multirow{3}{*}{$2.06\;(-5\%)$} & \multirow{3}{*}{$1.13\;(7\%)$} & \multirow{3}{*}{$0.79\;(-5\%)$} & \multirow{3}{*}{$1.57\;(29\%)$} & \multirow{3}{*}{$0.79\;(27\%)$} & \multirow{3}{*}{$0.59\;(26\%)$} & \multirow{3}{*}{$97.06$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{OnE}} & \multirow{3}{*}{$2.64\;(22\%)$} & \multirow{3}{*}{$1.4\;(32\%)$} & \multirow{3}{*}{$0.99\;(19\%)$} & \multirow{3}{*}{$2.04\;(67\%)$} & \multirow{3}{*}{$1.12\;(81\%)$} & \multirow{3}{*}{$0.77\;(64\%)$} & \multirow{3}{*}{$11.12$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\end{tabular}%
}
\label{table:Table2}
\end{table*}

==> paper SETA/Table3.tex <==
\begin{table*}[!htb]
\caption{Forecast performances on 2018, with the percentage variation with respect to Terna results between brackets.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{MAPE [\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAPE_{daily}[\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{dof}$}} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{Terna}} & \multirow{3}{*}{$2.41$} & \multirow{3}{*}{$1.14$} & \multirow{3}{*}{$0.9$} & \multirow{3}{*}{$1.65$} & \multirow{3}{*}{$0.76$} & \multirow{3}{*}{$0.62$} & \multirow{3}{*}{Unknown} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{OLS}} & \multirow{3}{*}{$2.74\;(14\%)$} & \multirow{3}{*}{$1.45\;(27\%)$} & \multirow{3}{*}{$1.07\;(19\%)$} & \multirow{3}{*}{$2.0\;(21\%)$} & \multirow{3}{*}{$0.99\;(30\%)$} & \multirow{3}{*}{$0.76\;(23\%)$} & \multirow{3}{*}{$9216$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TA}} & \multirow{3}{*}{$1.93\;(-20\%)$} & \multirow{3}{*}{$1.07\;(-6\%)$} & \multirow{3}{*}{$0.75\;(-17\%)$} & \multirow{3}{*}{$1.48\;(-10\%)$} & \multirow{3}{*}{$0.74\;(-3\%)$} & \multirow{3}{*}{$0.55\;(-11\%)$} & \multirow{3}{*}{$1569.78$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TS}} & \multirow{3}{*}{$1.93\;(-20\%)$} & \multirow{3}{*}{$1.07\;(-6\%)$} & \multirow{3}{*}{$0.75\;(-17\%)$} & \multirow{3}{*}{$1.49\;(-10\%)$} & \multirow{3}{*}{$0.74\;(-3\%)$} & \multirow{3}{*}{$0.55\;(-11\%)$} & \multirow{3}{*}{$406.03$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{RBF}} & \multirow{3}{*}{$1.92\;(-20\%)$} & \multirow{3}{*}{$1.06\;(-7\%)$} & \multirow{3}{*}{$0.74\;(-18\%)$} & \multirow{3}{*}{$1.46\;(-12\%)$} & \multirow{3}{*}{$0.73\;(-4\%)$} & \multirow{3}{*}{$0.55\;(-11\%)$} & \multirow{3}{*}{$80.49$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TE}} & \multirow{3}{*}{$\bf{1.87\;(-22\%)}$} & \multirow{3}{*}{$\bf{1.01\;(-11\%)}$} & \multirow{3}{*}{$\bf{0.72\;(-20\%)}$} & \multirow{3}{*}{$\bf{1.4\;(-15\%)}$} & \multirow{3}{*}{$\bf{0.68\;(-11\%)}$} & \multirow{3}{*}{$\bf{0.52\;(-16\%)}$} & \multirow{3}{*}{$114.5$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{OnE}} & \multirow{3}{*}{$2.32\;(-4\%)$} & \multirow{3}{*}{$1.22\;(7\%)$} & \multirow{3}{*}{$0.89\;(-1\%)$} & \multirow{3}{*}{$1.77\;(7\%)$} & \multirow{3}{*}{$0.89\;(17\%)$} & \multirow{3}{*}{$0.67\;(8\%)$} & \multirow{3}{*}{$4.15$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\end{tabular}%
}
\label{table:Table3}
\end{table*}

==> paper SETA/Table4.tex <==
\begin{table*}[!htb]
\caption{Forecast performances on 2019, with the percentage variation with respect to Terna results between brackets.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{MAPE [\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAPE_{daily}[\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{dof}$}} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{Terna}} & \multirow{3}{*}{$2.53$} & \multirow{3}{*}{$1.2$} & \multirow{3}{*}{$0.94$} & \multirow{3}{*}{$1.89$} & \multirow{3}{*}{$0.85$} & \multirow{3}{*}{$0.71$} & \multirow{3}{*}{Unknown} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{OLS}} & \multirow{3}{*}{$2.51\;(-1\%)$} & \multirow{3}{*}{$1.33\;(11\%)$} & \multirow{3}{*}{$0.98\;(4\%)$} & \multirow{3}{*}{$1.98\;(5\%)$} & \multirow{3}{*}{$0.92\;(8\%)$} & \multirow{3}{*}{$0.74\;(4\%)$} & \multirow{3}{*}{$9216$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TA}} & \multirow{3}{*}{$1.9\;(-25\%)$} & \multirow{3}{*}{$1.02\;(-15\%)$} & \multirow{3}{*}{$0.73\;(-22\%)$} & \multirow{3}{*}{$1.42\;(-25\%)$} & \multirow{3}{*}{$0.72\;(-15\%)$} & \multirow{3}{*}{$0.54\;(-24\%)$} & \multirow{3}{*}{$477.36$} \\ 
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TS}} & \multirow{3}{*}{$1.84\;(-27\%)$} & \multirow{3}{*}{$0.99\;(-18\%)$} & \multirow{3}{*}{$0.71\;(-24\%)$} & \multirow{3}{*}{$1.37\;(-28\%)$} & \multirow{3}{*}{$0.68\;(-20\%)$} & \multirow{3}{*}{$0.51\;(-28\%)$} & \multirow{3}{*}{$179.04$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{RBF}} & \multirow{3}{*}{$\bf{1.84\;(-27\%)}$} & \multirow{3}{*}{$\bf{0.99\;(-18\%)}$} & \multirow{3}{*}{$\bf{0.71\;(-24\%)}$} & \multirow{3}{*}{$\bf{1.36\;(-28\%)}$} & \multirow{3}{*}{$\bf{0.68\;(-20\%)}$} & \multirow{3}{*}{$\bf{0.51\;(-28\%)}$} & \multirow{3}{*}{$78.42$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{TE}} & \multirow{3}{*}{$1.91\;(-25\%)$} & \multirow{3}{*}{$1.04\;(-13\%)$} & \multirow{3}{*}{$0.74\;(-21\%)$} & \multirow{3}{*}{$1.48\;(-22\%)$} & \multirow{3}{*}{$0.73;(-14\%)$} & \multirow{3}{*}{$0.56\;(-21\%)$} & \multirow{3}{*}{$106.37$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\multirow{3}{*}{\thead{OnE}} & \multirow{3}{*}{$2.41\;(-5\%)$} & \multirow{3}{*}{$1.25\;(4\%)$} & \multirow{3}{*}{$0.92\;(-2\%)$} & \multirow{3}{*}{$1.88\;(-1\%)$} & \multirow{3}{*}{$0.97\;(14\%)$} & \multirow{3}{*}{$0.72\;(1\%)$} & \multirow{3}{*}{$3.71$} \\
& & & & & & & \\
& & & & & & & \\
\hline
\end{tabular}%
}
\label{table:Table4}
\end{table*}

==> paper SETA/Table5.tex <==
\begin{table*}[!htb]
\caption{Covariances, biases and Mean Squared Errors of RBF, TE and Terna forecasters, and the corresponding aggregated predictors.}
\centering %% in origine la dimensione era 0.6\columnwidth
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{2017}$}} & \multirow{3}{*}{\thead{$\mathbf{2018}$}} & \multirow{3}{*}{\thead{$\mathbf{2019}$}} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$Cov\left[e_{RBF}e_{Terna}\right]$}} & \multirow{3}{*}{$0.29$} & \multirow{3}{*}{$0.33$} & \multirow{3}{*}{$0.29$} \\ 
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$Cov\left[e_{TE}e_{Terna}\right]$}} & \multirow{3}{*}{$0.36$} & \multirow{3}{*}{$0.36$} & \multirow{3}{*}{$0.31$} \\ 
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$bias_{Terna}$}} & \multirow{3}{*}{$0.16$} & \multirow{3}{*}{$-0.52$} & \multirow{3}{*}{$-0.65$} \\ 
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$bias_{RBF}$}} & \multirow{3}{*}{$-0.03$} & \multirow{3}{*}{$0.02$} & \multirow{3}{*}{$-0.06$} \\ 
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$bias_{TE}$}} & \multirow{3}{*}{$-0.04$} & \multirow{3}{*}{$-0.01$} & \multirow{3}{*}{$-0.09$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$MSE_{Terna}$}} & \multirow{3}{*}{$1.13$} & \multirow{3}{*}{$1.29$} & \multirow{3}{*}{$1.43$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$MSE_{RBF}$}} & \multirow{3}{*}{$1.16$} & \multirow{3}{*}{$1.12$} & \multirow{3}{*}{$0.98$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$MSE_{TE}$}} & \multirow{3}{*}{$1.28$} & \multirow{3}{*}{$1.02$} & \multirow{3}{*}{$1.09$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$\hat{MSE}_{Avg(RBF)}$}} & \multirow{3}{*}{$0.72$} & \multirow{3}{*}{$0.77$} & \multirow{3}{*}{$0.75$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$MSE_{Avg(RBF)}$}} & \multirow{3}{*}{$0.71$} & \multirow{3}{*}{$0.77$} & \multirow{3}{*}{$0.77$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$\hat{MSE}_{Avg(TE)}$}} & \multirow{3}{*}{$0.78$} & \multirow{3}{*}{$0.76$} & \multirow{3}{*}{$0.79$} \\
& & & \\
& & & \\
\hline
\multirow{3}{*}{\thead{$MSE_{Avg(TE)}$}} & \multirow{3}{*}{$0.78$} & \multirow{3}{*}{$0.76$} & \multirow{3}{*}{$0.81$} \\
& & & \\
& & & \\
\hline
\end{tabular}%
}
\label{table:Table5}
\end{table*}

==> paper SETA/Table6.tex <==
\begin{table*}[!htb]
\caption{Aggregated forecast performances on 2017, with the percentage variation with respect to Terna results between brackets.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{MAPE [\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAPE_{daily}[\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE_{daily}[GW]}$}} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Terna}} & \multirow{3}{*}{$2.16$} & \multirow{3}{*}{$1.06$} & \multirow{3}{*}{$0.83$} & \multirow{3}{*}{$1.22$} & \multirow{3}{*}{$0.62$} & \multirow{3}{*}{$0.47$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(OLS)}} & \multirow{3}{*}{$1.87\;(-13\%)$} & \multirow{3}{*}{$0.96\;(-9\%)$} & \multirow{3}{*}{$0.72\;(-13\%)$} & \multirow{3}{*}{$1.19\;(-2\%)$} & \multirow{3}{*}{$0.6\;(-3\%)$} & \multirow{3}{*}{$0.45\;(-4\%)$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TA)}} & \multirow{3}{*}{$1.66\;(-23\%)$} & \multirow{3}{*}{$0.85\;(-20\%)$} & \multirow{3}{*}{$0.63\;(-24\%)$} & \multirow{3}{*}{$1.06\;(-13\%)$} & \multirow{3}{*}{$0.53\;(-15\%)$} & \multirow{3}{*}{$0.4\;(-15\%)$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TS)}} & \multirow{3}{*}{$1.66\;(-23\%)$} & \multirow{3}{*}{$0.85\;(-20\%)$} & \multirow{3}{*}{$0.63\;(-24\%)$} & \multirow{3}{*}{$1.04\;(-15\%)$} & \multirow{3}{*}{$0.52\;(-16\%)$} & \multirow{3}{*}{$0.39\;(-17\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(RBF)}} & \multirow{3}{*}{$\bf{1.66\;(-23\%)}$} & \multirow{3}{*}{$\bf{0.85\;(-20\%)}$} & \multirow{3}{*}{$\bf{0.63\;(-24\%)}$} & \multirow{3}{*}{$\bf{1.04\;(-15\%)}$} & \multirow{3}{*}{$\bf{0.52\;(-16\%)}$} & \multirow{3}{*}{$\bf{0.39\;(-17\%)}$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TE)}} & \multirow{3}{*}{$1.72\;(-20\%)$} & \multirow{3}{*}{$0.88\;(-17\%)$} & \multirow{3}{*}{$0.66\;(-20\%)$} & \multirow{3}{*}{$1.13\;(-7\%)$} & \multirow{3}{*}{$0.57\;(-8\%)$} & \multirow{3}{*}{$0.42\;(-11\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(OnE)}} & \multirow{3}{*}{$2.04\;(-6\%)$} & \multirow{3}{*}{$1.03\;(-3\%)$} & \multirow{3}{*}{$0.77\;(-7\%)$} & \multirow{3}{*}{$1.44\;(18\%)$} & \multirow{3}{*}{$0.76\;(23\%)$} & \multirow{3}{*}{$0.55\;(17\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\end{tabular}%
}
\label{table:Table6}
\end{table*}

==> paper SETA/Table7.tex <==
\begin{table*}[!htb]
\caption{Aggregated forecast performances on 2018, with the percentage variation with respect to Terna results between brackets.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{MAPE [\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAPE_{daily}[\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE_{daily}[GW]}$}} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Terna}} & \multirow{3}{*}{$2.41$} & \multirow{3}{*}{$1.14$} & \multirow{3}{*}{$0.9$} & \multirow{3}{*}{$1.65$} & \multirow{3}{*}{$0.76$} & \multirow{3}{*}{$0.62$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(OLS)}} & \multirow{3}{*}{$1.94\;(-20\%)$} & \multirow{3}{*}{$1.01\;(-11\%)$} & \multirow{3}{*}{$0.74\;(-18\%)$} & \multirow{3}{*}{$1.32\;(-20\%)$} & \multirow{3}{*}{$0.66\;(-13\%)$} & \multirow{3}{*}{$0.49\;(-21\%)$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TA)}} & \multirow{3}{*}{$1.71\;(-29\%)$} & \multirow{3}{*}{$0.88\;(-23\%)$} & \multirow{3}{*}{$0.65\;(-28\%)$} & \multirow{3}{*}{$1.16\;(-30\%)$} & \multirow{3}{*}{$0.58\;(-24\%)$} & \multirow{3}{*}{$0.43\;(-31\%)$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TS)}} & \multirow{3}{*}{$\bf{1.7\;(-29\%)}$} & \multirow{3}{*}{$0.87\;(-24\%)$} & \multirow{3}{*}{$0.65\;(-28\%)$} & \multirow{3}{*}{$\bf{1.15\;(-30\%)}$} & \multirow{3}{*}{$0.57\;(-25\%)$} & \multirow{3}{*}{$\bf{0.43\;(-31\%)}$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(RBF)}} & \multirow{3}{*}{$1.71\;(-29\%)$} & \multirow{3}{*}{$0.88\;(-23\%)$} & \multirow{3}{*}{$0.65\;(-28\%)$} & \multirow{3}{*}{$1.16\;(-30\%)$} & \multirow{3}{*}{$0.58\;(-24\%)$} & \multirow{3}{*}{$0.43\;(-31\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TE)}} & \multirow{3}{*}{$1.72\;(-29\%)$} & \multirow{3}{*}{$\bf{0.87\;(-24\%)}$} & \multirow{3}{*}{$\bf{0.65\;(-28\%)}$} & \multirow{3}{*}{$1.18\;(-28\%)$} & \multirow{3}{*}{$\bf{0.57\;(-25\%)}$} & \multirow{3}{*}{$0.44\;(-29\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(OnE)}} & \multirow{3}{*}{$1.9\;(-21\%)$} & \multirow{3}{*}{$0.96\;(-16\%)$} & \multirow{3}{*}{$0.72\;(-20\%)$} & \multirow{3}{*}{$1.34\;(-19\%)$} & \multirow{3}{*}{$0.67\;(-12\%)$} & \multirow{3}{*}{$0.5\;(-19\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\end{tabular}%
}
\label{table:Table7}
\end{table*}

==> paper SETA/Table8.tex <==
\begin{table*}[!htb]
\caption{Aggregated forecast performances on 2019, with the percentage variation with respect to Terna results between brackets.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 \textbf{} & \multirow{3}{*}{\thead{$\mathbf{MAPE [\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE [GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAPE_{daily}[\%]}$}} & \multirow{3}{*}{\thead{$\mathbf{RMSE_{daily}[GW]}$}} & \multirow{3}{*}{\thead{$\mathbf{MAE_{daily}[GW]}$}} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Terna}} & \multirow{3}{*}{$2.53$} & \multirow{3}{*}{$1.2$} & \multirow{3}{*}{$0.94$} & \multirow{3}{*}{$1.89$} & \multirow{3}{*}{$0.85$} & \multirow{3}{*}{$0.71$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(OLS)}} & \multirow{3}{*}{$1.95\;(-23\%)$} & \multirow{3}{*}{$0.99\;(-18\%)$} & \multirow{3}{*}{$0.74\;(-21\%)$} & \multirow{3}{*}{$1.45\;(-23\%)$} & \multirow{3}{*}{$0.69\;(-19\%)$} & \multirow{3}{*}{$0.54\;(-24\%)$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TA)}} & \multirow{3}{*}{$1.76\;(-30\%)$} & \multirow{3}{*}{$0.89\;(-26\%)$} & \multirow{3}{*}{$0.67\;(-29\%)$} & \multirow{3}{*}{$1.28\;(-32\%)$} & \multirow{3}{*}{$0.63\;(-26\%)$} & \multirow{3}{*}{$0.48\;(-32\%)$} \\ 
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TS)}} & \multirow{3}{*}{$1.73\;(-32\%)$} & \multirow{3}{*}{$0.88\;(-27\%)$} & \multirow{3}{*}{$0.65\;(-31\%)$} & \multirow{3}{*}{$1.23\;(-35\%)$} & \multirow{3}{*}{$0.6\;(-29\%)$} & \multirow{3}{*}{$0.46\;(-35\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(RBF)}} & \multirow{3}{*}{$\bf{1.73\;(-32\%)}$} & \multirow{3}{*}{$\bf{0.88\;(-27\%)}$} & \multirow{3}{*}{$\bf{0.65\;(-31\%)}$} & \multirow{3}{*}{$\bf{1.23\;(-35\%)}$} & \multirow{3}{*}{$\bf{0.6\;(-29\%)}$} & \multirow{3}{*}{$\bf{0.46\;(-35\%)}$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(TE)}} & \multirow{3}{*}{$1.78\;(-30\%)$} & \multirow{3}{*}{$0.9\;(-25\%)$} & \multirow{3}{*}{$0.67\;(-29\%)$} & \multirow{3}{*}{$1.3\;(-31\%)$} & \multirow{3}{*}{$0.64\;(-25\%)$} & \multirow{3}{*}{$0.49\;(-31\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\multirow{3}{*}{\thead{Avg(OnE)}} & \multirow{3}{*}{$1.98\;(-22\%)$} & \multirow{3}{*}{$1.0\;(-17\%)$} & \multirow{3}{*}{$0.75\;(-20\%)$} & \multirow{3}{*}{$1.51\;(-20\%)$} & \multirow{3}{*}{$0.74\;(-13\%)$} & \multirow{3}{*}{$0.57\;(-20\%)$} \\
& & & & & & \\
& & & & & & \\
\hline
\end{tabular}%
}
\label{table:Table8}
\end{table*}

==> paper SETA/Table9.tex <==
\begin{table}[ht]
\caption{Easter holiday dates: years 1990-2019.}
\centering %% in origine non c'era il resizebox
\resizebox{0.35\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
 \textbf{Year} & \textbf{Date} \\
 \hline
 $1990$ & April 12 - April 16 \\
 \hline
 $1991$ & March 28 - April 1 \\
 \hline
 $1992$ & April 16 - April 20 \\
 \hline
 $1993$ & April 8 - April 12 \\
 \hline
 $1994$ & March 31 - April 4 \\
 \hline
 $1995$ & April 13 - April 17 \\
 \hline
 $1996$ & April 4 - April 8 \\
 \hline
 $1997$ & March 27 - March 31 \\
 \hline
 $1998$ & April 9 - April 13 \\
 \hline
 $1999$ & April 1 - April 5 \\
 \hline
 $2000$ & April 20 - April 24 \\
 \hline
 $2001$ & April 12 - April 16 \\
 \hline
 $2002$ & March 28 - April 1 \\
 \hline
 $2003$ & April 17 - April 21 \\
 \hline
 $2004$ & April 8 - April 12 \\
 \hline
 $2005$ & March 24 - March 28 \\
 \hline
 $2006$ & April 13 - April 17 \\
 \hline
 $2007$ & April 5 - April 9 \\
 \hline
 $2008$ & March 20 - March 24 \\
 \hline
 $2009$ & April 9 - April 13 \\
 \hline
 $2010$ & April 1 - April 5 \\
 \hline
 $2011$ & April 21 - April 25 \\
 \hline
 $2012$ & April 5 - April 9 \\
 \hline
 $2013$ & March 28 - April 1 \\
 \hline
 $2014$ & April 17 - April 21 \\
 \hline
 $2015$ & April 2 - April 6 \\
 \hline
 $2016$ & March 24 - March 28 \\
 \hline
 $2017$ & April 13 - April 17 \\
 \hline
 $2018$ & March 29 - April 2 \\
 \hline
 $2019$ & April 18 - April 22 \\
 \hline
\end{tabular}%
}
\label{table:Table9}
\end{table}
